Learning Degradation Representations for Image Deblurring

In various learning-based image restoration tasks, such as image denoising and image super-resolution, the degradation representations were widely used to model the degradation process and handle complicated degradation patterns. However, they are less explored in learning-based image deblurring as blur kernel estimation cannot perform well in real-world challenging cases. We argue that it is particularly necessary for image deblurring to model degradation representations since blurry patterns typically show much larger variations than noisy patterns or high-frequency textures.In this paper, we propose a framework to learn spatially adaptive degradation representations of blurry images. A novel joint image reblurring and deblurring learning process is presented to improve the expressiveness of degradation representations. To make learned degradation representations effective in reblurring and deblurring, we propose a Multi-Scale Degradation Injection Network (MSDI-Net) to integrate them into the neural networks. With the integration, MSDI-Net can handle various and complicated blurry patterns adaptively. Experiments on the GoPro and RealBlur datasets demonstrate that our proposed deblurring framework with the learned degradation representations outperforms state-of-the-art methods with appealing improvements. The code is released at https://github.com/dasongli1/Learning_degradation.

==> figs/gopros.tex <==
\setlength{\tabcolsep}{2pt}
\begin{figure*}[ht]
    \small
    \begin{center}
    \begin{tabular}{ccccccc}
        \includegraphics[width=.48\linewidth]{figs/supp/410_132_input.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/410_132_gt.png} & \\
        Blurry & Reference \\ 
        \includegraphics[width=.48\linewidth]{figs/supp/410_132_hinet1.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/410_132_ours1.png} & \\
        HINet \cite{HINet} & Ours \\
        \includegraphics[width=.48\linewidth]{figs/supp/410_167_input.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/410_167_gt.png} & \\
        Blurry & Reference \\ 
        \includegraphics[width=.48\linewidth]{figs/supp/410_167_hinet1.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/410_167_ours1.png} & \\
        HINet \cite{HINet} & Ours \\
        
        % GT & 1-d code & Using $L_1$ loss & Ours\\
    \end{tabular}
    \end{center}
    \vskip -0.1in
    \caption{Image deblurring comparisons on the GoPro dataset \cite{deblur-multi-scale}. }
    \label{fig:gopro}
    % \vspace{-3mm}
\end{figure*}

==> figs/realblur.tex <==
\setlength{\tabcolsep}{2pt}
\begin{figure*}[h!]
    \small
    \begin{center}
    \begin{tabular}{ccccccc}
        \includegraphics[width=.48\linewidth]{figs/supp/205a-input.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/205a-gt.png} & \\
        Blurry & Reference \\ 
        \includegraphics[width=.48\linewidth]{figs/supp/205a-hinet1.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/205a-ours1.png} & \\
        HINet \cite{HINet} & Ours \\
        \includegraphics[width=.48\linewidth]{figs/supp/208a-input.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/208a-gt.png} & \\
        Blurry & Reference \\ 
        \includegraphics[width=.48\linewidth]{figs/supp/208a-hinet1.png} &
        \includegraphics[width=.48\linewidth]{figs/supp/208a-ours1.png} & \\
        HINet \cite{HINet} & Ours \\
        
        % GT & 1-d code & Using $L_1$ loss & Ours\\
    \end{tabular}
    \end{center}
    \vskip -0.1in
    \caption{Image deblurring comparisons on the RealBlur dataset \cite{realblur}. }
    \label{fig:realblur}
    % \vspace{-3mm}
\end{figure*}
